Accelerating Sparse DNNs Based on Tiled GEMM

Network pruning can reduce the computation cost of deep neural network (DNN) models. However, sparse models often produce randomly-distributed weights to maintain accuracy, leading to irregular computations. Consequently, unstructured sparse models cannot achieve meaningful speedup on commodity hardware built for dense matrix computations. Accelerators are usually modified or designed with structured sparsity-optimized architectures for exploiting sparsity. For example, the Ampere architecture introduces a sparse tensor core, which adopts the 2:4 sparsity pattern. We propose a pruning method that builds upon the insight that matrix multiplication generally breaks the large matrix into multiple smaller tiles for parallel execution. We present the tile-wise sparsity pattern, which maintains a structured sparsity pattern at the tile level for efficient execution but allows for irregular pruning at the global scale to maintain high accuracy. In addition, the tile-wise sparsity is implemented at the global memory level, and the 2:4 sparsity executes at the register level inside the sparse tensor core. We can combine these two patterns into a tile-vector-wise (TVW) sparsity pattern to explore more fine-grained sparsity and further accelerate the sparse DNN models. We evaluate the TVW on the GPU, achieving averages of $1.85\times$, $2.75\times$, and $22.18\times$ speedups over the dense model, block sparsity, and unstructured sparsity.

==> tex/analysis.tex <==
\begin{figure}[t]
    \begin{center}
        % \vspace{-3mm}
    \includegraphics[width=1\columnwidth]{figures/methods.pdf}
    \caption{Comparison of three patterns with 50\% sparsity: element-wise (\benchmark{EW}) pattern prunes individual elements, vector-wise (\benchmark{VW}) pattern prunes half elements in a 4-element vector, and block-wise (\benchmark{BW}) pattern prunes an entire $2\times 2$ block.}
    \label{fig:pruning_patterns}
    \end{center}
    %\vspace*{-.4cm}
\end{figure}

\vspace*{0.2cm}
\section{Pruning Efficiency Analysis} 
\label{sec:analysis}

In this section, we study the impact of different DNN pruning algorithms on the model execution efficiency.
Network pruning can remove the excessive weights in DNN models, and therefore the resulted sparse model has less weight size and computation cost.
However, our analysis shows that the sparse models generated by existing pruning algorithms cannot achieve meaningful speedup on the dense architectures.


\subsection{Sparsity Pattern}

There are two major components in the algorithms for pruning deep neural networks. The first component is how to evaluate the importance of individual weight element (i.e., importance score). And the second component is the sparsity pattern that is removed altogether.
In this part, we mainly focus on the study of different sparsity patterns, and we explain the details of importance score calculation in \Sec{sec:pruning_algorithm}.

\Fig{fig:pruning_patterns} illustrates different sparsity patterns.
The first sparsity pattern, called \benchmark{element-wise (EW)}, removes the individual weight element solely by its importance score rank. 
For instance, prior work~\cite{han2015learning} proposes to remove weight elements with small magnitude.
This approach imposes no constraints on the sparsity pattern and could remove most of weights among all pruning methods.
Thus, it is also called unstructured pruning.
However, the randomly distributed non-zero weights lead to substantial irregular memory accesses, which imposes great challenges for efficient hardware execution.
As such, researchers propose other two more structured pruning methods.

The second sparsity pattern shown in the middle of \Fig{fig:pruning_patterns}, called \benchmark{vector-wise (VW)}~\cite{zhu2019sparse,yao2019balanced}, divides a column in the weight matrix to multiple vectors.
Within each vector, it prunes a fixed portion of elements by the rank of their importance scores.
This approach preserves the randomness within each vector for model accuracy.
Meanwhile, it also maintains the regular structure  for efficient execution, where different vectors have the same number of non-zero weight elements.
The third pattern, called \benchmark{block-wise (BW)}~\cite{narang2017block}, divides the weight matrix to small blocks, and treats a block as the basic pruning unit. 
In other words, the \benchmark{EW} sparsity pattern is a special case of  the \benchmark{BW} sparsity pattern, which expands a $1\times 1$ block to an $n \times n$ block.
The structural sparsity pattern \benchmark{BW} leads to the efficient execution of sparse models. 



	\begin{figure}[t]
    \begin{subfigure}{0.48\columnwidth}
	% \vspace*{-.2cm}
	\includegraphics[trim=0 0 0 0, clip, width=.9\linewidth]{figures/sparsity_vgg}
	    %\vspace*{-.2cm}
    \caption{VGG.}
    \label{fig:sparsity_vgg}
    \end{subfigure}~
    \begin{subfigure}{0.48\columnwidth}
    % \vspace*{-.2cm}
	\includegraphics[trim=0 0 0 0, clip,  width=.9\linewidth]{figures/sparsity_bert}
	    %\vspace*{-.2cm}
    \caption{BERT.}
    \label{fig:sparsity_bert}
    \label{fig:pattern_b}
    \end{subfigure}
	%   \vspace*{-.2cm}
	\caption{Sparsity and execution time comparison between dense and various sparse models (VGG and \hlc{BERT}). \hlc{The accuracy of various sparse models is 1\% lower than the dense model.}}
	\label{fig:sparsity_compare}
	    \vspace*{-.4cm}
	\end{figure}

\subsection{Execution Efficiency Analysis}

We first use two popular deep neural network models to evaluate the execution efficiency of sparse models generated by the aforementioned three sparsity patterns.
Our experimental results show that although these pruning approaches can lead to sparse models with a large volume of sparsity (i.e., zero weight elements), they fail to achieve a meaningful speedup compared to the unmodified dense model on the existing GPUs. 
Moreover, the emergence of dense matrix multiplication accelerators such as tensor core further widens their performance gap.
 
We first study a CNN model VGG-16~\cite{simonyan2015very} with 13 convolutional layers and 3 fully connected layers. 
We evaluate it on the image classification task using the ImageNet dataset~\cite{krizhevsky2017imagenet}.
The second studied model is BERT (base) in \Sec{background:bert}, which is a Transformer-based model with 12 encoding layers.
We evaluate the BERT model with the sentence classification task on the MNLI dataset~\cite{wang2019glue}.
We use the vector size of 16 for \benchmark{VW} and the block size of $32\times32$ for \benchmark{BW} as suggested in their original papers~\cite{zhu2019sparse,narang2017block}.
% We prune both models with the three different sparsity patterns and keep the accuracy drop of each model within 2\% of its unmodified dense version.

We perform the efficiency analysis on a V100 GPU~\cite{volta2017whitepaper} with CUDA 10.1~\cite{nvidia2019toolkit}. 
Besides the CUDA cores, the V100 GPU also integrates the specialized tensor core for the acceleration of dense matrix multiplication.
This GPU has a peak throughput of 15.7 TFLOPS (floating point operation per second) and 125 TFLOPS for the CUDA cores and tensor cores, respectively. 
We evaluate the performance of dense model with the cuDNN library on the CUDA core and tensor core separately.
We execute the sparse model of \benchmark{EW} and \benchmark{VW} with the cuSparse~\cite{nvidia2019toolkit} library, which executes only on the CUDA cores.
We execute the sparse model of \benchmark{BW} with the BlockSparse~\cite{blocksparse2020} library, which leverages the tensor cores owing to its regularity.

\Fig{fig:sparsity_compare} compares the sparsity and performance between the dense and sparse models with various patterns. 
All patterns achieve over 50\% sparsity with the greatest by \benchmark{EW}.
The performance of \benchmark{EW} and \benchmark{VW} is slower than their dense version on the CUDA core (Dense-C). 
In addition, the performance gap between the dense model and sparse model exacerbates when the dense matrix accelerator tensor core is used (Dense-T).
Prior work~\cite{zhu2019sparse} reports a $1.5\times$ speedup using the \benchmark{VW} pattern, which requires non-negligible modifications of the tensor core.
\benchmark{BW} achieves the best performance among all sparse models as it runs on the tensor core.
However, its performance is still $3\times$ slower than the dense model on the tensor core.

  In summary, the existing pruning approaches generate sparse models that are inefficient on the existing hardware.
As such, we need a sparsity pattern that can match the existing hardware features while maintaining fine granularity, which is critical for achieving high model accuracy.



==> tex/methodology.tex <==
\section{methodology} \label{sec:methodology}
\subsection{Cutalss}
\subsection{Optimization for BERT (Transpose, Kernel fusion)}
\subsection{Tricks on pruning (multi-stages, ...)}
\subsubsection{multi-stages}
Our implementation is based on the hierarchically blocked structuresCUTLASS\cite{cutlass2019} for GEMM. 
Compared to pruning lots of weights in one time, and fine tune with many epoches, we find that the performance of pruning few weights time by time and fine tune few epoches will be better. For example, if the final sparsity is 40\%, the accuracy of pruning 40\% weights and fine-tuning three epoches is 82.12\%, but the accuracy of pruning 20\% weights in first time and prune 10\% weight in other times and fine-tuning one epoch after each pruning is 82.52\%. 

\subsubsection{Consider whole network v.s. consider layer by layer}

Different pruning region for each time is also leads to different performance. If we compute the scores of all layers, and prune the lower score weights on whole network, the accuracy would be better. But the reduction of FLOP would be worse. For example, if we prune 50\% on both K and N dimension, the ideal FLOP reduction ratio is 75\%. But the real reduction ratio in our experiment is about 69\%. On the other hand, if we compute the score and prune the lower score weights layer by layer, then the FLOP reduction ratio will be 75\% as we expect, but the accuracy would be worse. 



==> tex/related.tex <==
\section{Related Work and Discussion}
\label{sec:related_work}


\paragraph{Architectural Support for Sparse DNN.}
Recently, designing efficient architectures for sparse DNN models has become an active research topic. There are many prior works to dealing with sparsity through architectural support~\cite{hua2019boosting, zhang2019eager, deng2019tie, yang2019sparse, hegde2019extensor, sadi2019efficient}. ExTensor~\cite{hegde2019extensor} proposes a novel approach to accelerate tensor algebra kernels using the principle of hierarchical computation elimination in the presence of sparsity. Sparse ReRAM Engine~\cite{yang2019sparse} exploits both the weight and activation sparsity to accelerate the DNN model. The channel gating~\cite{hua2019boosting} is a fine-grained dynamic pruning technique for CNN inference. Those work are all based on customized ASIC or FPGA. 
There are also prior works~\cite{guo2020balancing_arxiv,zhu2019sparse} that focus on optimizing the tensor core for better performance or flexibility.

\paragraph{Software Optimization for Sparse DNN.}
There are also previous works that propose software optimization for sparse model acceleration on modern architectures without hardware modification.
Prior work proposes an efficient mixed-mode representation called MM-CSF for sparse tensor, which partitions nonzero elements into disjoint sections for performance acceleration~\cite{nisa2019efficient}. 
CFS SpMV is a new optimization strategy for the sparse matrix-vector multiplication and shows high performance on multicore architectures~\cite{elafrou2019conflict}.  DCSR (densified compressed sparse row) is well-suited to GPU architecture for sparse computation using the near-memory strategy~\cite{fujiki2019near}.

\paragraph{\proj{} on Other Platforms.}
 Although we only implement \proj{} on the GPU platform, it is quite possible to support our sparsity pattern on other platforms like TPU~\cite{jouppi2017datacenter}. 
    The fundamental requirement of supporting \proj{} is the medium size GEMM.
Our evaluation shows that \proj{} with $G=128$ strikes a balance between model accuracy and latency, which implies the requirement of $128\times N \times128$ GEMM.
    The latest TPU~\cite{tpuv2} adopts a relatively large systolic array ($128 \times 128$), which meets the aforementioned requirement.
    However, it only exposes high-level programming interfaces like GEMM, which makes the other optimization like streaming concurrency difficult. 
    In other words, supporting \proj{} on other platforms like TPU is feasible if their low-level programming interfaces are exposed.
    
\paragraph{Sparsity Patterns.}
The sparsity pattern plays an important role in both the model accuracy and architecture design for sparse DNNs.
Zhu et al. propose the vector-wise pruning pattern and the corresponding sparse tensor core architecture~\cite{zhu2019sparse}.
The vector-wise pruning pattern adds constraints on the sparsity of each pruning unit to guarantee the pruned matrices to be acceleration-friendly.
They reported accuracy results on popular CNN and RNN models.
However, this method fails to capture the uneven sparsity distribution across different model layers, which limits its pruning effect.
Narang et al. propose the block-wise pruning pattern~\cite{narang2017block}.
This pattern has the prune unit as a block, making it execution-friendly on the dense GPU architecture.
However, their method has a strong constraint on the pruning shape which impacts the model accuracy significantly.

Recent work also explores energy-oriented pruning, targeting both accelerators~\cite{yang2018energy, yang2017designing} and general-purpose processors~\cite{yang2018ecc, yang2018netadapt}. Our work removes redundant computations and thus could also reduce energy consumption. Yang et al.~\cite{yang2020automatic} demonstrate quantization-pruning joint compression.
